A Hybrid mmWave and Camera System for Long-Range Depth Imaging

mmWave radars offer excellent depth resolution even at very long ranges owing to their high bandwidth. But their angular resolution is at least an order-of-magnitude worse than camera and lidar systems. Hence, mmWave radar is not a capable 3-D imaging solution in isolation. We propose Metamoran, a system that combines the complimentary strengths of radar and camera to obtain accurate, high resolution depth images over long ranges even in high clutter environments, all from a single fixed vantage point. Metamoran enables rich long-range depth imaging with applications in security and surveillance, roadside safety infrastructure and wide-area mapping. Our approach leverages the high angular resolution from cameras using computer vision techniques, including image segmentation and monocular depth estimation, to obtain object shape. Our core contribution is a method to convert this object shape into an RF I/Q equivalent, which we use in a novel radar processing pipeline to help declutter the scene and capture extremely weak reflections from objects at long distances. We perform a detailed evaluation of Metamoran's depth imaging capabilities in 400 diverse scenes. Our evaluation shows that Metamoran estimates the depth of static objects up to 90 m and moving objects up to 305 m and with a median error of 28 cm, an improvement of 13$\times$ compared to a naive radar+camera baseline and 23$\times$ compared to monocular depth estimation.

==> intro-2.tex <==
\section{Introduction}

% In this paper, we seek to build high-resolution depth images for scenes with objects at distances of   meters. Depth imaging at a long range has been an ongoing challenge in the computer vision community, for applications such as autonomous navigation, industrial IoT and surveillance. Prior literature in this space has been unable to reliably complete long-range depth imaging due to limited range (e.g. stereo[] or monocular[] depth imaging), poor resilience to ambient light (e.g. LIDAR) or poor angular resolution (e.g. radar systems). We focus on two solutions, both relatively low-cost and popular on automotive platforms: cameras and automotive radars. These two solutions are quite complementary in their strengths and weaknesses -- radar provides resilience against environmental effects and excellent range resolution (3.75 cm at 100 meters) -- about 10 times better than camera systems, however their angular resolution is at least 10 times poorer than camera systems. This naturally leads us to the question -- ``Can we fuse the existing cameras and radar sensor data on vehicles to provide the best of both worlds?''


% Finally, millimeter wave (mmWave) RADARs are also popularly used on autonomous cars to detect and range targets while being resilient to fog, rain and snow []. While they provide excellent range resolution(3.75cm), their angular resolutions are far from that of a LiDAR (0.1 degree). At best, with large antenna arrays [], mmWave RADARs can provide 1 degree azimuth resolutions. At long ranges (50-100m), even 1 degree azimuth beamwidth can lead to poor shape resolution, as seen in Figure . To add to this, RADAR images often suffer from many spurious peaks (see Figure. ).

One of the most appealing features of mmWave radar systems arises from its high bandwidth and carrier frequency, which enables precise depth estimation at long depth ranges, often as large of 60 meters, and at cm-scale resolutions. This finds application in a wide range of areas, including security~\cite{bjorklund2012evaluation}, automobile safety~\cite{wenger1998automotive}, industrial sensing and control~\cite{dandu2021high}.
%mmWave radars have been widely deployed in varied contexts, including security~\cite{bjorklund2012evaluation}, automobile safety~\cite{wenger1998automotive}, industrial sensing and control~\cite{dandu2021high}. Due to the high bandwidth of mmWave radio frequencies, mmWave radars have an excellent depth resolution -- at few tens of centimeters over distances as much as 60 meters. 
For comparison, most RGB camera solutions of the same physical form-factor (e.g. monocular depth estimation~\cite{bhat2020adabins}, depth cameras~\cite{zed2}, stereo-vision~\cite{smolyanskiy2018importance}, etc.) struggle to reach such resolutions for objects at extended distances and are about an order-of-magnitude worse. Yet, mmWave radars, by themselves, are not a capable 3-D imaging solution as their angular resolution along both azimuth and elevation is extremely poor --- with the best radars of the market at least 10$\times$ poorer than camera systems. This has led to mmWave radars being restricted to niche applications -- for instance, in airport security~\cite{bjorklund2012evaluation} or physical collision sensing~\cite{wenger1998automotive} ---  where their impressive depth range and resolutions are not fully utilized. This naturally leads us to the question: \textit{Can we fuse cameras and mmWave radar sensor data  to provide the best of both worlds and build a rich 3-D depth imaging solution?}. 
%
In doing so, we seek a 3-D imaging system that can be readily deployed from a single fixed vantage point to enable applications as long-range road-side safety systems, surveillance and security applications, wide-area mapping and occupancy sensing. 


% In this paper we ask the question: How can we fuse readily available camera and mmWave radar sensors to get better than the best of both worlds? At face value, it is trivial that using both a camera and a mmWave radar would provide better results, as cameras struggle with depth information at a long range (\~100m) and mmWave radars have poor angular resolution. However, what if the fusion of both of these sensors resulted in better depth information than a mmWave alone could provide, and angular detection of objects that a camera alone could not see?

This paper presents \name\footnote{A fictional race from the Dragon Ball Universe that taught Son Goku the Fusion technique~\cite{metamoran}. }, a hybrid mmWave and camera-based sensing system that achieves high angular and depth resolution for objects at significant distances -- up to 60 meters (see Fig.~\ref{fig:main}). It achieves this through a \textit{novel specular radar processing algorithm} that takes
%\acsnote{didnt follow whtat "feeds as priors" means} 
information from computer vision algorithms such as deep neural network-based image segmentation as input. While efforts have been made to fuse radar and camera data in the past, primarily for short range object detection and tracking \cite{chang2020spatial}, imaging under physical \cite{palffy2019occlusion} or weather-related occlusions \cite{liu2021robust}, this paper considers the unique problem of hybrid mmWave/camera sensing for long-range outdoor depth imaging. 

%\name\ is evaluated on a large dataset of mmWave radar and camera data from fixed vantage points across diverse outdoor locations in a major U.S. city. 


% While efforts have been made to fuse radar and cameras in the past, these have focused on occlusion resilience, including limited field-of-view[], weather-related occlusions[], and movement[]. We instead are targeting the issue of range resolution at a distance. We also have the privilege of building upon large bodies of work in wireless sensing algorithms[] and camera processing algorithms[], but we distinguish ourselves from this body of work by focusing on fusion.


\begin{figure*}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.8\textwidth, height=6cm]{figures/systemoverview.PNG}
        \vspace*{-0.1in}
    \captionof{figure}{\textbf{\name}\ devises a novel mmWave specular beamforming algorithm that forms high resolution depth-images 60~m away from objects-of-interest, using inputs from vision techniques such as image segmentation. }
    \label{fig:main}
\end{figure*}


A key contribution in our system
%\acsnote{challenge ? sounds more like a contribution} 
is improving depth sensing capabilities beyond what is typically achievable by a mmWave radar alone using a novel radar processing algorithm that provides high depth resolution (along the $z$-axis) \textit{guided} by computer vision techniques that have high spatial resolution (in $x$ and $y$).
%In theory, the depth resolution of a mmWave radar is quite good (few decimeters), but because of its limited angular resolution, objects close to each other can become merged as a single object.
% due to insufficient variation in azimuth or elevation angle.
%Furthermore, this reduced resolution results in a blurred capture of the object's outline and shape. In contrast, cameras have precisely the opposite problem --- the high-angular resolution results in fairly precise object outlines, but their depth resolution is poor.
%
%Our key insight is therefore combining the high spatial ($x$ and $y$) resolution of camera imaging with the high depth resolution (in $z$) of mmWave radars. 
%
First, we detect and identify an object using a camera-based image segmentation algorithm, which gives us the angular position (in the $x$-$y$ plane)  of objects in the environment as well as their spatial outline. 
%
Our key technical contribution is a novel specular radar beamforming algorithm (see Sec.~\ref{sec:beamform}) that returns high-resolution depth estimates by processing radar signals along the angular span and shape outline for each  object in the image identified using segmentation. We then show how such a system could be combined with dense monocular depth estimates to create robust depth images of individual objects, capturing depth variation within the object itself, even at extended distances away from the radar-camera platform. In other words, we show how semantic inferences on vision data collected by the camera can help declutter and provide useful priors to obtain high-resolution depth images that are better than standalone radar or camera algorithms. 

Our second contribution is to address various challenges in making \name\ robust in case of cluttered environments, unfavorable object orientation, extended distances and partial occlusions that impede the radar, camera, or both. We address this problem specifically for stationary objects: this form radar's worst-case scenario (Doppler can help to detect moving objects) as objects that are not moving (e.g. traffic signs, parked cars, children at a bus stop) can also be important to detect. %For mobile objects with extremely weak radar reflections (e.g. cars or pedestrians at extended distances), we exploit their mobility to perform background subtraction to isolate their spatial depths from significant distances. 
We narrow down objects whose spatial bounds are consistent across both camera and radar images, thereby allowing for increased robustness by reducing clutter. We also observe strong reflections from out-of-spatial bound reflectors leak into our spatial bound of interest and design cancellation techniques to detect weak reflections which would otherwise be masked by spurious objects. Further, we design and show how \name\ continues to operate well, even amid partial occlusions, e.g. due to fog or partial occlusion from other objects. We document instances where radar systems can actively be used to improve camera image segmentation by identifying objects that were initially missed by segmentation. 

% \name\ can be further enhanced through another opportunity -- using the observations from radar physics to refine our learning based computer vision models. In particular, we seek to use mmWave depth observations to further refine image segmentation. For example, in the case of a person occluded by a curtain, the mmWave radar would provide multiple depths for the curtain despite only the curtain being detected by the camera. Furthermore, the high range resolution of mmWave can help to identify objects narrowly separated in range and at a much higher resolution than cameras are capable of. With the assistance of depth information, image processing algorithms can geometrically narrow down the possible positions of occluded objects, monitor movement, and continuously track reflectors moving in and out of view. The addition of mmWave can be used to refine detection of occluded objects, further detailed in section XXX.

We implement \name\ with a TI MMWCAS-RF-EVM radar and a FLIR Blackfly S 24.5MP color camera. Due to the relative lack of rich public mmWave radar I/Q datasets over long distances, we collected extensive data (200 scenes totalling 100 GB of I/Q samples and camera data) in diverse scenes outdoors at a major U.S. city. Both \name's source code and datasets will be made \textbf{open source} upon paper acceptance to benefit the community. A few highlights from our results include:
\begin{itemize}[leftmargin=*]
\item An evaluation of the effective median depth of an object-of-interest at distances of up to 60 meters, in diverse outdoor settings, at a median error of 28 cm. This is  an improvement of about 23$\times$ versus state-of-the-art monocular depth estimation and 13$\times$ versus a naive camera + radar beamforming solution. 
\item Dense estimation of the azimuthal/depth profile of a single object-of-interest, for an imaging error of 80 cm at distances up to 60 meters. This is an improvement of about 4$\times$ versus state-of-the-art monocular depth estimation and 6$\times$ versus a naive camera + radar beamforming solution.
%A study of the distribution of depth errors of individual pixels within the object of interest with significant improvements over state-of-the-art. 
% 80 cm accurate median depth imaging of objects-of-interest at distances up to 60 meters  an improvement of about 4$\times$ versus state-of-the-art monocular depth estimation and 6$\times$ versus a naive camera + radar beamforming solution. \acsnote{How is this bullet different from previous one}
\item A demonstration of resilience to various classes of partial occlusions and blockages. %and poor weather conditions (e.g. fog
\end{itemize}


\sssec{Contributions:} We makes the following contributions.
\begin{itemize}[leftmargin=*]
    \item \name, a novel system that combines camera and mmWave sensing to achieve high resolution depth images at long ranges. 
    \item A specular beamforming algorithm that leverages the output of image segmentation algorithms from computer vision to declutter and retrieve depths of objects-of-interest from radar I/Q samples. 
 \item A detailed implementation and evaluation of \name\ in varied environments to demonstrate substantial improvements in long range depth imaging. 
 \end{itemize}
 
 \sssec{Limitations:} We concede that our system is limited by more significant occlusions that impact camera observations and discuss the limitations of our system in Sec.~\ref{sec:limitations} as well as present an evaluation of both successful and failure modes with various types of occlusions in our results in Sec.~\ref{sec:results}. 



%Autonomous navigation requires a complete understanding of the 3D environment. Today, high fidelity 3D images provide essential input to path planning and perception engines. However, they generate large volumes of data at a slow update rate of 5-20 Hz []. This raises problems [] for short-term, highly-critical decision making engines such as ... While some of these problems are solved by a high update rate RGB camera, associating depth information not only improves performance in these problems [] but also provides solution when a 2D image is fundamentally insufficient []. Thus, a 3D sensor providing quick updates is an invaluable asset for a system designer engineering safe autonomous navigation. 

%We note that for most tasks, it is sufficient to obtain depth maps of a certain object/s in a scene, and not the whole scene []. Truncating the scene to objects' specific spatial coordinates, gets rid of spurious peaks and makes it easier to improve RADAR images. Truncating RADAR images is not so trivial. Blobby images no longer hold any resemblance to the objects' shapes and RADAR image interpretation becomes hard. On the other hand, RGB cameras, which are also pervasive in autonomous navigation [], have been shown to detect real world objects [] and provide semantic meaning to the scene []. On top of object detection, given the resolution of modern cameras, it's possible to estimate the object's azimuth and elevation coordinates []. We now introduce our solution, \textit{\name}, which fuses camera and RADAR images by understanding the scene from a camera and using it to improve RADAR images. 

%While \name's image truncation helps scene understanding and removes unwanted peaks, truncated image is still blobby and needs to be sharpened. An image is blobby either because its dimensions are comparable to the spatial resolutions, or the truncated scene is crowded and reflections from each object superimpose, or because of properties of radio wave propagation along multiple paths from RADAR to object and back which lead to unintended objects appearing in the truncated image (see Figure ). \name\ tackles each of these issues systematically. Upon object detection, by carefully guessing the object shape and dimensions from the camera image, \name\ casts the problem of sharpening RADAR image as a sparse recovery problem of extracting the presence of a candidate object/s in a blobby RADAR image. Section xx details this algorithm.

%Our contribution is an algorithm design using a fusion of camera and mmWave RADAR signals in order to provide quick, high resolution depth maps to help tackle short-term highly critical problems. ....

%\name\ is implemented end-to-end using commodity off the shelf automotive RADAR AWR1843 and RGB camera FLIR xxx. We benchmark the performance of our system, accuracy at long ranges and system update rate, against a Realsense depth camera, a mechanical LiDAR, raw mmWave depth estimates and recent systems improving mmWave RADAR images.  







==> intro-3.tex <==
\section{Introduction}

Modern security cameras are tasked with identifying objects of interest and observing if they violate any regulations. Depending on the use case, they maybe used to monitor if people enter no-clearance area in corporate buildings and warehouses, drones enter no-fly zone on top of certain buildings, or if unwanted objects enter large agriculture fields. These applications would require the cameras to detect, classify and estimate depth of objects at long ranges, ideally from a single vantage point so that the system is easy to deploy. While the performance of state-of-the-art algorithms vary for each of the tasks at long ranges, depth estimation (e.g: monocular depth estimation ~\cite{bhat2020adabins}) gives meters of error for objects beyond 10-20 m. On the other hand, lidar which by default measures depth is marketed to reach 100 meters range. But in practical deployments, we observed it's accurate to only about 30 meters vastly dependent on sunlight and size of objects. In this paper, we ask what does the sensor suite and algorithms look like in the next generation long range security \textit{cameras}. 

Apart from cameras and lidars, another mainstream depth sensor today is the mmWave radar. One of the most appealing features of mmWave radar systems arises from its high bandwidth, which enables precise depth estimation at long ranges, often as large as 100 meters, and at cm-scale resolutions. This finds application in a wide range of areas, including security~\cite{bjorklund2012evaluation}, automobile safety~\cite{wenger1998automotive}, industrial sensing and control~\cite{dandu2021high}. Yet, mmWave radars, by themselves, are not a capable 3-D imaging solution as their angular resolution along both azimuth and elevation is extremely poor --- with the best radars of the market at least 10$\times$ poorer than camera systems. With poor angular resolutions, peaks due to different objects can easily be confused and cannot be effectively identified. This has led to mmWave radars being restricted to niche applications -- for instance, in airport security~\cite{bjorklund2012evaluation} or physical collision sensing~\cite{wenger1998automotive} ---  where their impressive operating range and resolutions are not fully utilized. We make a key observation that radars and cameras are mutually complementary in terms of angular resolution and depth estimation at long ranges. This naturally leads us to the question: \textit{Can we fuse cameras and mmWave radar sensor data to provide the best of both worlds and build a rich 3-D depth imaging solution?}. 

This paper presents \name\footnote{A fictional race from the Dragon Ball Universe that taught Son Goku the Fusion technique~\cite{metamoran}. }, a hybrid mmWave and camera-based sensing system that achieves high angular and depth resolution for objects at significant distances -- up to 90 meters (see Fig.~\ref{fig:main}). It achieves this through a \textit{novel radar processing algorithm} that takes information from computer vision algorithms such as deep neural network-based image segmentation as input to produce precise depth estimation. While efforts have been made to fuse radar and camera data in the past, primarily for short range object detection and tracking \cite{chang2020spatial}, imaging under physical \cite{palffy2019occlusion} or weather-related occlusions \cite{liu2021robust}, this paper considers the unique problem of hybrid mmWave radar and camera sensing for long-range depth imaging. 


\begin{figure*}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.8\textwidth, height=6cm]{figures/systemoverview.PNG}
        \vspace*{-0.1in}
    \captionof{figure}{\textbf{\name}\ devises a novel mmWave specular beamforming algorithm that forms high resolution depth-images 60~m away from objects-of-interest, using inputs from vision techniques such as image segmentation. }
    \label{fig:main}
\end{figure*}

A key challenge in designing a radar and camera fusion system is identifying which reflections from the radar heatmap correspond to the objects of interest. One of the main contributors is the poor radar angular resolution because of which the radar signature of objects might not resemble the shape of the object in the real world. Because of this objects can't be directly identified from radar heatmap, but owing to camera's superior angular sensing abiliies, computer vision techniques such as image segmentation can guide the radar to search over particular angular spans to find the object. Despite this, searching over this assumes the shape is easily discernible across the segmented heatmap. While this might be true for large extended objects such as trucks at long ranges, objects such as car and persons look like a few points on the radar heatmap. On top of this, the radar signature's intensity is affected at long ranges and depends highly on the reflective characteristics of the object. Due to all these reasons, the objects' reflection will be present but very weak. Our technical contribution is a novel radar beamforming algorithm (see Sec.~\ref{sec:beamform}) informed by camera data that finds the weak signal and returns high-resolution depth estimates. The idea is to use monocular depth estimation of the segmented object. While the absolute depth estimate will be off at long ranges, the depth profile of an object such as car will be accurate []. In this way, we construct a shape contour of what the object should look like if radar had very high resolution. Our algorithm generates a radar signature template corresponding to this shape contour and searches across the segmented heatmap to find the object. Once the absolute depth estimates are obtained, we then show how such a system could be combined with monocular depth estimates to create depth images of individual objects, capturing depth variation within the object itself, even at extended distances away from the radar-camera platform. In other words, we show how semantic inferences on vision data collected by the camera can help declutter and provide useful priors to obtain high-resolution depth images that are better than standalone radar or camera algorithms. 

Our second contribution is to address various challenges in making \name\ robust in case of cluttered environments and partial occlusions that impede the camera. We observe certain reflections originating from (buildings, fences, electric poles) outside the segmented angles have strong side lobes and leak into the segmented signal of interest. This causes clutter which makes the search process prone to a lot of false positives. Similarly, partial occlusions which block portions of the objects of interest also create unintended signatures which might lead to false positives sheerly because they are strong reflections. To tackle this we design techniques similar to successive intereference cancellation [] which essentially removes the clutter and helps with accurate depth estimation. Both strong out-of-interest reflectors and partial occluders are first identified and eliminated successively.

In addition to depth sensing, next generation security cameras would need robust image segmentation and classification. Image segmentation gets confused when the object and the scene lack colour contrast and object is partially occluded. While camera helped radar with depth imaging, we believe radar can help improve the confidence of camera image segmentation and classification as well. Radar signatures at long ranges are very weak, but at short ranges can provide meaningful information such as approximate size and reflectivity characteristics (metal or non metal) of objects. This can be used to disambiguate between objects and conditionally change the image segmentation and classification confidences.


We implement \name\ with a TI MMWCAS-RF-EVM radar and a FLIR Blackfly S 24.5MP color camera. Due to the relative lack of rich public mmWave radar I/Q datasets over long distances, we collected extensive data (200 scenes totalling 100 GB of I/Q samples and camera data) in diverse scenes outdoors at a major U.S. city. \name's datasets will be made \textbf{open source} upon paper acceptance to benefit the community. A few highlights from our results include:
\begin{itemize}[leftmargin=*]
\item An evaluation of the effective median depth of an object-of-interest at distances of up to 60 meters, in diverse outdoor settings, at a median error of 28 cm. This is  an improvement of about 23$\times$ versus state-of-the-art monocular depth estimation and 13$\times$ versus a naive camera + radar beamforming solution. 
\item Dense estimation of the azimuthal/depth profile of a single object-of-interest, for an imaging error of 80 cm at distances up to 60 meters. This is an improvement of about 4$\times$ versus state-of-the-art monocular depth estimation and 6$\times$ versus a naive camera + radar beamforming solution.
%A study of the distribution of depth errors of individual pixels within the object of interest with significant improvements over state-of-the-art. 
% 80 cm accurate median depth imaging of objects-of-interest at distances up to 60 meters  an improvement of about 4$\times$ versus state-of-the-art monocular depth estimation and 6$\times$ versus a naive camera + radar beamforming solution. \acsnote{How is this bullet different from previous one}
\item A demonstration of resilience to various classes of partial occlusions and blockages. %and poor weather conditions (e.g. fog
\end{itemize}


\sssec{Contributions:} We makes the following contributions.
\begin{itemize}[leftmargin=*]
    \item \name, a novel system that combines camera and mmWave sensing to achieve high resolution depth images at long ranges. 
    \item A specular beamforming algorithm that leverages the output of image segmentation algorithms from computer vision to declutter and retrieve depths of objects-of-interest from radar I/Q samples. 
 \item A detailed implementation and evaluation of \name\ in varied environments to demonstrate substantial improvements in long range depth imaging. 
 \end{itemize}
 
 \sssec{Limitations:} We concede that our system is limited by more significant or complete occlusions that impact camera observations and discuss the limitations of our system in Sec.~\ref{sec:limitations} as well as present an evaluation of both successful and failure modes with various types of occlusions in our results in Sec.~\ref{sec:results}. 







==> intro.tex <==
\section{Introduction}

Title: Fast, depth maps at long range using COTS sensors

Autonomous navigation requires a complete understanding of the 3D environment. Today, high fidelity 3D images provide essential input to path planning and perception engines. But, they generate large volumes of data at a slow update rate of 5-20 Hz []. This raises problems [] for short-term, highly-critical decision making engines such as ... While some of these problems are solved by a high update rate RGB camera, associating depth information not only improves performance in these problems [] but also provides solution when a 2D image is fundamentally insufficient []. Thus, a 3D sensor providing quick updates is an invaluable asset for a system designer engineering safe autonomous navigation.  

Passive depth sensors using stereo configurations [] and structured light projection based depth sensors [] only provide limited range of operation [] and sacrifice depth accuracy for compactness and portability []. Time of flight LiDARs have emerged as the ubiquitous choice of accurate 3D sensors for long range applications such as driving on roads [] and navigating through open factory floors []. Mechanically steered LiDARs, although operating at extremely long ranges ($>$ 100 m), provide slow update rate owing to mechanical steering []. However, optical phased arrays provide better update rate (... Hz) but are not shown to work at ranges $>$ 20m []. Current sensor solutions lack the ability to provide quick (100s of Hz), high fidelity depth information at long ranges ($\sim$ 100m).

In addition to LiDARs, millimeter wave (mmWave) RADARs are also popularly used on autonomous cars to detect and range targets while being resilient to fog, rain and snow []. mmWave RADARs, operating in radio frequencies suffer lesser power attenuation compared to visible/infrared frequencies used in LiDARs, thereby allowing long range target detection. However, commodity RADARs today are far from being a panacea. While they provide excellent range-independent range resolutions (3.75cm) owing to high system bandwidths (4GHz), and provide very high (kHz) update rates, their azimuth (14 degrees) and elevation resolutions are far from that of a LiDAR (0.1 degree). Most recent hardware techniques comprising of large antenna arrays [], providing 1 degree azimuth resolutions, have opened the door for true 3D RADAR imaging. RADAR imaging holds promise for obtaining fast, long range and accurate depth estimates. But, at long ranges (50-100m), even 1 degree azimuth beamwidth can lead to RADAR images to be very blobby, as seen in Figure . To add to this, RADAR images are often spluttered with spurious peaks (see Figure. ).

We note that for most tasks, it is sufficient to obtain depth maps of a certain object/s in a scene, and not the whole scene []. Truncating the scene to objects' specific spatial coordinates, gets rid of spurious peaks and makes it easier to improve RADAR images. Truncating RADAR images is not so trivial. Blobby images no longer hold any resemblance to the objects' shapes and RADAR image interpretation becomes hard. On the other hand, RGB cameras, which are also pervasive in autonomous navigation [], have been shown to detect real world objects [] and provide semantic meaning to the scene []. On top of object detection, given the resolution of modern cameras, it's possible to estimate the object's azimuth and elevation coordinates []. We now introduce our solution, \textit{\name}, which fuses camera and RADAR images by understanding the scene from a camera and using it to improve RADAR images. 

While \name's image truncation helps scene understanding and removes unwanted peaks, truncated image is still blobby and needs to be sharpened. An image is blobby either because its dimensions are comparable to the spatial resolutions, or the truncated scene is crowded and reflections from each object superimpose, or because of properties of radio wave propagation along multiple paths from RADAR to object and back which lead to unintended objects appearing in the truncated image (see Figure ). \name\ tackles each of these issues systematically. Upon object detection, by carefully guessing the object shape and dimensions from the camera image, \name\ casts the problem of sharpening RADAR image as a sparse recovery problem of extracting the presence of a candidate object/s in a blobby RADAR image. Section xx details this algorithm.

Our contribution is an algorithm design using a fusion of camera and mmWave RADAR signals in order to provide quick, high resolution depth maps to help tackle short-term highly critical problems. ....

\name\ is implemented end-to-end using commodity off the shelf automotive RADAR AWR1843 and RGB camera FLIR xxx. We benchmark the performance of our system, accuracy at long ranges and system update rate, against a Realsense depth camera, a mechanical LiDAR, raw mmWave depth estimates and recent systems improving mmWave RADAR images.  







==> method-old.tex <==
\section{Component Breakdown}\label{sec:primer}

\subsection{mmWave Radar}
Radars once only limited to military applications, are today used ubiquitously in a variety of applications from collision avoidance in autonomous driving~\cite{tokoro1996automotive}, to gesture recognition in smart phones~\cite{liu2020real} and industrial automation~\cite{mazgula2020ultra}. A key factor which enabled this trend was the usage of mmWave frequencies which allowed for compact antenna arrays and wide bandwidths, both of which are crucial for radars' target ranging and imaging capabilities. mmWave radars, as the name suggests, use radio waves of millimeter scale wavelengths in either 60 GHz (unlicensed band) or 77-81 GHz (autonomous vehicles band), by first actively illuminating an environment and then processing the reflections from various objects in the environment. This is noticeably different from modern image sensors which purely rely on passively sensing rays which make their way to the sensor. The reflections from the objects encode useful information such as objects' range, azimuth, elevation and velocity with respect to radar. The transmitted illumination and radar hardware are the main factors which limit the radars' ability to generate high resolution 3D images of the scene.

\sssec{Advantages of mmWave Radar: } Most commodity radars transmit a FMCW (Frequency Modulated Continuous Wave) signal which is  a waveform that continuously changes its frequency over time to span a significant bandwidth $B$. A radar's range resolution is fundamentally limited by this effective bandwidth of the transmitted signal as $\frac{c}{2B}$ ($c$ is speed of light). In the automotive band, we have a theoretical range resolution of 3.75 cm over tens of meters. In this regard, radars are on par with time of flight LIDARs which report typical range accuracies of 3 cm. Moreover, unlike LIDARs, radars work in all weather conditions (rain, snow, fog) and extreme ambient lighting (sunlight)~\cite{mullen2000hybrid}.


%Upon RF processing (see Figure~\ref{}), each reflected signal becomes a sinusoid with a frequency that is determined by its range and an initial phase corresponding to phase shift experienced by the signal during propagation ($\frac{4\pi d}{\lambda}$, where $\lambda$ is the wavelength of the signal and $d$ is the range). Applying a Discrete Fourier Transform (DFT) on the sinusoid, gives the range of the reflector. This also tells us that two reflectors can be distinguished only if they can be resolved by the DFT as two different frequencies. Thus, 


% The initial phase of sinusoids received across different antenna elements contain phase shifts which encode azimuth and elevation information. Standard radar processing once again involves applying Fourier transform across the antenna elements [] to obtain a 3D image of range, azimuth and elevation. This tells us that,

\sssec{Limitations of mmWave Radar: } But unfortunately radars have a poorer azimuth and elevation resolutions compared to both cameras and LIDARs. While range resolution is limited by the bandwidth of the  radar signal,  angular resolutions is dictated by the number of antenna elements that are packed on a radar. Greater the number of antenna elements, better the resolution. The best state-of-the-art automotive radar available~\cite{tiradar} with as many as 86x4 antenna elements has a 1.4$^{\circ}$x18$^{\circ}$ angular resolution. In contrast, state of the art LIDARs today also achieve 0.1$^{\circ}$x2$^{\circ}$, atleast 10x better angular resolution than radars~\cite{liu2008airborne}. With a poor angular resolution, 3D radar images look very coarse and blobby in the angular domain. While more antenna elements can be added, they come at significant increases in device cost and form-factor -- bridging the 10$\times$ gap is simply not an option with today's state-of-the-art hardware. We make the observation that even commodity cameras, because of their dense focal planar array image sensors, are better than radars in terms of angular resolution at about 0.02$^{\circ}$x0.02$^{\circ}$~\cite{napier2013cross}. This observation leads us to study combining the high angular resolution of camera systems with the high depth resolution of mmWave radar -- an approach we describe in the next section.

\subsection{Camera}
Cameras are of course ubiquitous in our modern world, but here we provide some context for the design decisions taken in selecting a camera for use in complementing a RADAR. FOV, megapixels

\subsection{Calibration}

We note that \name\ requires both internal calibration of the components as well as external calibration between the camera and the radar. 

Corner Reflector

Camera intrinsics & Fisheye removal

Externally, \name\ requires a consistent understanding of object shapes between the mmWave platform system and the camera system. While both of these are co-located in \name, they are at a small relative distance of XXX~cm, which could lead to inconsistencies in the images produced by the two modalities. \name\ accounts for this by performing a joint calibration step of the mmWave radar and camera using a feature-rich metallic surface that is viewed from both the camera and radar platform to capture a Euclidean transform between their frames of reference. The object is chosen to be feature-rich for both platforms, with stark differences in both color and the presence/absence of strong mmWave reflectors (metallic structures). We note that the transform obtained from calibration is applied, prior to fusing measurements from either platform to ensure consistency. 

\begin{figure}%[!htb]
\centering
\includegraphics[width=0.5\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{\name's Architecture:} \name\ uses image segmentation algorithms to find a shape along the x-y axes of each object-of-interest. It then applies super-resolution radar algorithms to refine the depth along the z-axis and depth completion algorithms to report an RGB-D output. }
\vspace*{-0.1in}
\label{fig:arch}
\end{figure}

\section{\name's Approach}
\name\ at a high level, takes as input camera and 77~GHz mmWave radar data from a common scene. We use these inputs to fuse and return a high-resolution depth image for specific objects of interests including cars and persons at distances of several tens of meters away. Our key contribution is a novel radar processing algorithm that produces refined depth estimates for specific objects of interest, based on priors obtained through semantic segmentation of camera images. We choose a radar-based processing approach rather than an exclusive deep-learning based approach on all underlying data (images + raw I/Q), due to better explainability of the inferences. Besides, the resolution obtained from our system in depth is close to the physical limits that can be obtained owing to the bandwidth of the radar. Nevertheless, our solution benefits heavily from state-of-the-art deep neural network based semantic segmentation algorithms that operate on image data. 

\sssec{System Architecture and Outline: } Fig.~\ref{fig:arch} depicts the architecture of our system that we elaborate in the following sections. First, we apply two state-of-the-art pre-processing steps that operate on image data  (Sec.~\ref{sec:semseg}): (1) Semantic segmentation, i.e. identify the spatial (x and y) bounds of objects-of-interest -- cars and people; (2) Monocular depth estimation to obtain an approximate estimate for the shape of these objects, albeit prone to error at large distances. We then design a novel specular beamforming algorithm in Sec.~\ref{sec:beamform} that uses priors along one dimension (x and y) from semantic segmentation and monocular depth estimate which provide a coarse shape of the object of interest to then obtain a fine-grained depth estimate. (3) Our final step (Sec.~\ref{sec:depthcomp}) is to combine the sparse inferred depth values from \name's mmWave processing with camera image data through state-of-the-art depth completion algorithms~\cite{zhao2020adaptive}, refined from prior art on LIDAR depth completion, to obtain a high-resolution RGB-D images for objects of interest in the scene. 


\section{Image Pre-Processing}\label{sec:semseg} 

\name's first step is to process camera image data to learn about the approximate span in azimuth and elevation of  objects-of-interest, as well as an approximate silhouette or outline along the x-y plane, i.e. parallel to the depth axis. We specifically consider two specific classes of objects-of-interest that are important in autonomous driving -- cars and pedestrians. As mentioned in Sec.~\ref{sec:primer}, we exploit the high angular resolution of camera systems that are at about 0.02$^{\circ}$x0.02$^{\circ}$~\cite{napier2013cross} --  orders-of-magnitude better than mmWave radar systems. \name's vision pre-processing steps below are therefore crucial in providing prior information on the shape and location of objects-of-interest along the x-y plane so that mmWave data can be used to focus on these objects and improve resolution along the z-axis. 


% Why does camera have good angular resolution (azimuth and elevation)? By looking at the perspective project equations of a focal plane array camera sensor when passing through a simple lens (\url{http://www.cse.psu.edu/~rtc12/CSE486/lecture12.pdf} - slide 13). $x = f\frac{X}{Z}; y = f\frac{Y}{Z} => x = f tan(\theta) ; y = f tan(\phi)$
%\url{https://github.com/facebookresearch/detectron2}


\begin{figure}%[!htb]
\centering
\includegraphics[width=0.5\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{Image Segmentation:} \name\ uses image segmentation to identify the spatial bounds along the x-y axes of objects-of-interest -- cars and pedestrians --  with semantic labels assigned. }
\vspace*{-0.1in}
\label{fig:panoptic}
\end{figure}


\subsection{Image Segmentation} 

To identify the spatial bounds (along x-y) of objects of interest, we perform state-of-the-art image segmentation which labels objects by their type and plots masks that capture the outline of these objects -- an example of which is shown in Fig.~\ref{fig:panoptic}. 


We perform image segmentation using Detectron2 \cite{wu2019detectron2} trained with KITTI dataset. This model has been previously trained on cars and pedestrians -- the two classes of objects that we consider. We use both of these types of objects as our primary test subjects without additional model tuning. Image segmentation provides a segmentation mask (outline) and instance ID of each detected object as shown in Fig.~\ref{fig:panoptic}. The segmentation mask directly provides the spatial bounds and precise shape of the object along the x-y plane and is fed as a prior for mmWave specular beamforming in Sec.~\ref{sec:beamform} below.

%Works well for cars and people, so we used those as the primary test subjects. As well as applicability.


\subsection{Monocular Depth Estimation} 

As a second step, we perform state-of-the-art monocular depth estimation specifically on objects-of-interest filtered through image segmentation above. We use this scheme both as a baseline for comparison and to provide a coarse range of depths that the object spans. We use AdaBins~\cite{bhat2020adabins} for monocular depth estimation of the objects of interest as detected by the image segmentation step. We note that state-of-the-art monocular depth estimation is poor in terms of accuracy and resolution at extended distances, with errors of about XXX meters and resolution of XXX m at distances of about 80 meters. Nevertheless, we observe that monocular depth estimation provides  useful prior information on the approximate range of depths that the object spans and an approximate 3-D shape (outline) of the object that serve as useful priors for our  mmWave specular beamforming algorithm in Sec.~\ref{sec:beamform} below.


%\url{https://arxiv.org/pdf/2011.14141v1.pdf}

%{Find some information/citations on what kind of situations monocular depth estimation works well in: ideally, bad at ranging but good at depth calculation}

%Used to decide shape for specular beamforming




\section{Vision-improved Detection} \label{sec:detection}

Improving the ability of a mmWave radar to detect and find the range of a given reflector falls into three broad categories: reducing false positive rate from spurious peaks and unwanted reflectors, increasing the ability of our system to detect weak reflectors, and providing resilience to occlusions. We discuss how the introduction of a camera allows \name\ to improve in all of these categories when compared to radar alone.

\begin{figure*}%[!htb]
\centering
\includegraphics[width=\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{\name\ vs. Radar Beamforming:} A qualitative comparison of the depth images generated by \name\ versus standard radar beamforming that tends to be coarse in spatial resolution. }
\vspace*{-0.0in}
\label{fig:mmwavebeamform}
\end{figure*}


\begin{figure*}%[!htb]
\centering
\includegraphics[width=\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{\name\ vs. Monocular Depth Estimation:} \name\ could enhance both absolute and relative errors in the depth distribution within an object-of-interest using monocular depth estimation by using measurements from the mmWave radar.  }
\vspace*{-0.0in}
\label{fig:monoculardepth}
\end{figure*}

\subsection{Clutter Reduction} To improve the robustness of \name's algorithm, we present a key optimization that was pivotal in identifying the true depth of objects-of-interest. In particular, our focus is in cluttered environment where reflections from a large number of objects impede identifying the depth of the true object. At first blush, one might assume that even with a large number of objects in the environment, the number of objects at the desired azimuth and elevation angle -- as specified by semantic segmentation, would be relatively few. Further, given that the object is in direct line-of-sight of the camera, it can also be expected to correspond to the first peak observed along this 3-D angle. 

In practice, however, peaks corresponding to extremely strong reflectors in the environment result in significantly large spots in the radar image, with their size mainly due to the poor angular resolution of radar. These spots often leak into a significant range of azimuths and elevation, resulting in spurious objects detected at distances, often closer than the object-of-interest. More problematically, such spots could also be the result of objects of a similar shape (e.g. another car). Fortunately, however, these spots are easy to label as not from an objects-of-interest, as long as they are centered at different azimuth or elevation values. One must therefore perform a de-clutter phase prior to applying \name's specular beamforming algorithm that discounts and eliminates spurious results at depths that correspond to these spurious peaks. Doing so would prevent \name's algorithm from being misled by such peaks. Fig.~\ref{fig:mmwavebeamform} provides a qualitative comparison of the impact of \name's algorithm in de-cluttering the radar image and identifying the true peak.

\sssec{Correcting Absolute Errors: } To address the first challenge, we can simply shift the monocular depth estimates for any given object-of-interest so that they line up with the estimate from \name's specular beamforming algorithm. This ensures that absolute errors for any given object-of-interest are minimized. A key point to note is that for large objects (e.g. a car), there may be some ambiguity on which exact point on the monocular depth estimate should be shifted to line up with \name's estimate. To remedy this, we correlate the object template used in Sec.~\ref{sec:depth} from semantic segmentation with the image that resulted from monocular depth estimation. Recall that this very object template was used to estimate the object's depth in \name's super-resolution algorithm. The correlation process therefore allows us to identify the pixel on the image that best corresponds with the depth estimates from \name's super-resolution algorithm. 

\sssec{Correcting Relative Errors: }To address the second challenge of dealing with errors in monocular depth estimation, one can fine-tune \name's specular beamforming algorithm to zoom in on depths of parts of the object-of-interest. Specifically, one could extend \name's algorithm in Sec.~\ref{sec:depth} to compute object depth at finer resolution by trivially modifying the object template to center at different azimuth and elevation values, as desired, within the spatial bounds of the object as defined by image segmentation. These can be further refined to follow specific bands-of-interest of monocular depth estimation whenever depth estimation confidence is low. In effect, this would result in a unique depth value from mmWave signal data that can be obtained along each azimuth and elevation queried through the camera image that is a fusion of monocular depth imaging and mmWave sensing. 


\subsection{Detecting Weak Reflections}  

Traditionally, doppler

In this section, we explore ways to amplify extremely weak reflections from objects-of-interest, either due to their material properties, poor orientation or extended range from the radar. Indeed, the precise level to which radar reflections weaken depends on a combination of all of these properties and we evaluate this further for a diverse set of objects in Sec.~\ref{sec:microbenchmarks}. While in most instances, isolating weak reflections from static objects is challenging, two classes of common objects of interest in autonomous driving -- pedestrians and vehicles are often mobile.

\name\ can therefore use background subtraction to isolate reflections off moving objects -- essentially capturing multiple I/Q samples across two different time instances and subtracting the two to isolate reflections from moving objects. This greatly reduces background clutter and improves the signal-to-noise ratio of mobile objects in the environment. While background subtraction is common in radar systems in general~\cite{}, one could directly combine it with \name's approach that fuses observations with image data. Specifically, we can simultaneously perform semantic segmentation on two consecutive image snapshots \textit{as well as} background subtraction on radar data to identify which objects in the image have moved. At this point, one can then perform \name's algorithm on the subtracted I/Q samples across snapshots to better isolate the depths of objects-of-interest. Fig.~\ref{fig:bgsub} presents an example of an instance where background subtraction significantly helped identify the depth of an object that was completely mis-identified in its absence.  



\subsection{Resilience to Partial Occlusions}  

Use camera to determine what is in front of object, remove peak if it is a known object magnitude, find two peaks and take the further one if it is an unknown magnitude

\name\ is also designed to be robust to partial occlusions such as fog or physical obstructions. While in some instances of partial obstructions, semantic segmentation can be fairly robust, it could fail in other instances. However, mmWave radars are known to be fairly resilient to partial occlusions, especially fog~\cite{guan2020through}. To remain robust to instances where semantic segmentation may miss an object-of-interest, \name\ also annotate depths at objects with strong dominant peaks in the radar image, even if not specifically flagged as vehicle or pedestrian during semantic segmentation. For these objects identified through radar, we nevertheless feed in (partial) shape outlines if available from monocular depth estimation or semantic segmentation. Fig.~\ref{fig:occlusions} is a representative example of instances where our approach succeeds in estimating depths of objects that are missed by semantic segmentation and our discussion in Sec.~\ref{sec:limitations} also captures failure modes of this approach, especially for severe occlusions (e.g. heavy fog). 

\subsection{Algorithm}

\name's specular beamforming algorithm process the complex I/Q samples received from the mmWave radar platform, coupled with the shape outlines of objects of interest in the scene, obtained from the image pre-processing steps in Sec.~\ref{sec:semseg} above. In traditional mmWave beamforming~\cite{steinhauer2008millimeter}, received I/Q samples are effectively projected along all spatial angles (azimuth and elevation) to obtain the signal time-of-arrival between the object to the radar. This quantity, when multiplied by the speed of light to obtain the depth of the object. Unfortunately, this approach relies on the azimuth resolution of the radar, which is fundamentally limited by the number of antennas on the radar itself -- at best $1.4^\circ$ in state-of-the-art radar systems. The end result is a coarse radar image as shown in Fig.~\ref{fig:mmwavebeamform}(a). 


\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \caption{Specular Beamforming Algorithm}
    \Input{Spatial Bounds S of object-of-interest O_i
    \\Monocular Depth Estimates d_m of O_i  
    \\Wireless channel measurements h at radar
    \\ Virtual antenna array positions $X_a = x_1, x_2, .. x_n$ of radar}
    \Output{Depth Image D(x,y)}
    
    $\For {(r, \theta), \theta \in S$}{
    
    for 
    $(x, y) = polar2cart(r, \theta)$
    $x = x + X_a$
    $dist = \sqrt(x^2 + y^2) + dmr$
    
    }
    
    
    $R_{mask}(x,y) = 1~~~  \forall (x,y)| (||(x,y)-R_{optimal}||_2 < ||(x,y)-R||_2 \forall R\neq R_{optimal})$
    $(\mathbf{X},\mathbf{Y})_{allowed} = (\mathbf{X},\mathbf{Y})_{allowed} .* R_{mask}$\;
    $P(x,y) = 0~~\forall (x,y)\in(\mathbf{X},\mathbf{Y})_{allowed}$\;
    \For{each $(BS^m, BS^n)$ pair}{$tdoaMeasured^{m,n} = \underset{t}{argmax}~~ InverseNDFT(\mathbf{\tilde{h}}, \mathbf{f})$}
    $tdoaActual^{m,n} = tdoaMeasured^{m,n} + tdoaRef_{R_{optimal}}^{m,n}$\;
    % \For{each $BS^m$ $\epsilon$ $\mathbf{BS}$}{
    %     Estimate $dist(C,BS^m)$ using $(\frac{P_{t}}{P_{r}})_{dB} = -20*log_{10}\frac{dist(C,BS^m)}{dist(R_{optimal},BS^m)}$
    % }
    % \For{$(x,y)$ $\epsilon$ $(\mathbf{X},\mathbf{Y})_{allowed}$}{
    %     \For{each $(BS^m, BS^n)$ pair}{
    %         $z = | ||(x,y)-BS^m||_2 - ||(x,y)-BS^n||_2 - tdoaActual^{m,n} |$\;
    %         \uIf{$z < mar$}{$P(x,y) = P(x,y) + e^{-z/2\sigma^2}$}
    %     }
    % }
    \textbf{return} ParticleFilter($(\mathbf{X},\mathbf{Y})_{allowed}$, GetProbability)\;
    \tcc{Run Particle filter~\cite{van2001unscented} sampling allowed space using GetProbability(.)}
    
    
    
    
        \SetKwFunction{FMain}{GetProbability}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$x, y$}}{
        \For{each $(BS^m, BS^n)$ pair}{
            \uIf{$z = | ||(x,y)-BS^m||_2 - ||(x,y)-BS^n||_2 - tdoaActual^{m,n} | <  mar / \text{Penalty}(x,y)$}{$P(x,y) = P(x,y) + e^{-z/2\sigma^2}$}
        }
        }

    \label{algm:al}
\end{algorithm}



\sssec{Detailed Algorithm: }Mathematically, \name's algorithm uses the approximate shape outline inferred from image pre-processing, coupled with a mmWave ray-tracing model to estimate the expected I/Q samples of reflections from such an object -- i.e. the \text{object template}. Of course, these I/Q samples would in practice experience a phase-shift due to the unknown distance of the object-of-interest from the radar, with a distance of $d$ resulting in a phase shift of exactly $4 \pi d / \lambda$, where $\lambda$ is the signal wavelength. \name\ then applies a matched-filter to obtain $P(d)$ -- the correlation of the object template at each possible depth $d$ relative to the radar. We then report the range of this object as the value of $d$ with that corresponds to the maximum of $P(d)$. Algorithm~\ref{algm:al} provides a more elaborate description of the steps of \name\ for FMCW mmWave radar signals. 

\begin{figure*}%[!htb]
\centering
\includegraphics[width=\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{\name\ vs. Partial Occlusions:} \name\ can help identify objects-of-interest despite partial occlusions and improve semantic segmentation by pointing to missed objects.  }
\vspace*{-0.0in}
\label{fig:occlusions}
\end{figure*}

\section{Vision-improved Imaging}
\subsection{Intra-Object Depth Profiling}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth, height=0.15\textheight]{figures/SystemDiagram.png}
\vspace*{-0.1in}
\caption{\textbf{Picture of some combination of LIDAR output, depth image output, RADAR output, radar + depth}}
\vspace*{-0.1in}
\end{figure}

We note our current description of \name's algorithm provides only one depth value per object template, i.e. one depth per object. However, in practice, we would require multiple depth values across the range of pixels within the object. In an ideal world, we would like an output similar to monocular depth estimation (see Fig.~\ref{fig:monoculardepth} for an example). In monocular depth estimation, pixel color and other image features are used to identify objects at various depth levels resulting in an RGB-D image at multiple depth bands as shown in Fig.~\ref{fig:monoculardepth}. However two problems persist in such an image: (1) First, while monocular depth estimation may often correctly return the \textit{relative} depths between different parts of a large object such as a car, it often makes large errors in \textit{absolute} depths, particularly for objects at extended distances~\cite{}. (2) Second, monocular depth estimation often struggles with objects that do not have significant variation in color or sharp edges that simplify depth estimation~\cite{}.  The rest of this section describes how we address both these challenges to obtain \name's depth images (see Fig.~\ref{fig:monoculardepth}) that offer superior accuracy to monocular depth estimation. 

==> overview.tex <==
\section{Overview}

==> related-old.tex <==
\section{Related Work}
\textbf{Wireless Sensing: }Recent years have seen extensive work in sensing the environment using wireless communication radios. Past work has leveraged variations in Wi-Fi signals for applications including imaging~\cite{Huang2014, DepatlaAPM17} and location tracking~\cite{Xie:2015:PPD:2789168.2790124, SpotFi}. Perhaps most closely related to our work are recent material detection systems~\cite{Wu2016,TagScan,LiquID} that can detect material by sensing how signals are attenuated by objects placed between the transmitter and receiver. Much of this work assumes multiple access points or bulky infrastructure in the environment and are therefore ill-suited for mobile platforms such as UAVs.

This work instead seeks to discover the location and material of multiple potentially occluded objects in the environment using moving Wi-Fi radios on a mobile platform without supporting infrastructure. Further, we seek to sense the environment, not characteristics of a UAV as in~\cite{Tam}. Finally, we distinguish ourselves from~\cite{karanam20173d}, in that we seek to sense the environment via reflections rather than penetrations.

\textbf{Sensing Alternatives to Commodity Wireless:} RADAR systems use synthetic aperture radar polarimetry for topography imaging~\cite{Praks2009,536542,7770718,rs9060560}. Aircraft and satellites can even use polarization of received RADAR signals to measure soil moisture of farmland~\cite{shi1997estimation}. Recent years has seen the polarimetry largely unchanged as a sensing modality but used with new materials~\cite{metasurfaces} and for new applications~\cite{arctic}. Building on this work, we seek to bring radar polarimetry to light-weight commodity Wi-Fi cards. To accomplish this, we face challenges such as the near-far effect, imperfections of such radios, and shorter proximity than an airplane or a satellite, where polarimetry systems are commonly deployed.

Cameras~\cite{mejias2010vision}, LIDARs~\cite{ramasamy2016lidar} and depth imaging~\cite{huang2017visual} are often used to detect objects, for instance by autonomous vehicles and UAVs. While these  sense obstacles in direct field of view, they fail to detect objects that are occluded (e.g. hidden pedestrian or drones around the corner) -- a challenge commodity wireless can address. Furthermore, they struggle with to measure depth at a high resolution at long range, achieving meter-scale accuracy at up to 80m range in monocular depth estimation cases\cite{Zhao_2020} and only operating up to around 20m in the case of depth cameras\cite{zed2}.

\textbf{Fusion of RF and Camera:} Camera and RF fusion based approaches are proposed for automatic re-calibration \cite{xu2012towards}, industrial workplace \cite{savazzi2015device}, and fall detection \cite{kianoush2016device}. Alahi et al. ~\cite{alahi2015rgb}  proposed to estimate depth of a user using WiFi RSSI and associate it with an RGB image captured through a camera for localizing the individual. Fang et al. ~\cite{fang2020eyefi} fuses motion trajectory from WiFi CSI and camera for person identification and tracking. 


\textbf{Fusion of Camera and Depth and RADAR: } There exist many works that explore fusion with cameras with RADAR to provide a complementary sensing system. One use is for attention selection: using RADAR to detect objects of interest to reduce computational load\cite{Ji2008}. Another application of these systems is to fill the blind spots between camera and RADAR: using cameras to detect things like lines on the road and object boundaries, and using RADAR in poor weather conditions and to detect depth\cite{Kato2002}.
SO-NET \cite{john2019so} integrates semantic segmentation and object detection in a joint multitask framework by fusing monocular camera and RADAR. The results show that the fusion based approach performs superior in perception tasks than vision-only based approach. Siyang at el. \cite{han2016frontal} proposed a perception system for intelligent cars to fuse a mmWave RADAR and a monocular camera for detecting frontal objects in roads, which can be useful for Advanced Driver Assistant Systems (ADAS). In the proposed method, the RADAR based detections are converted to regions of interest (ROI) first. Then, these ROIs are classified by four classifiers (vehicles, pedestrians, two wheels, traffic cones) using Deformable Part Model (DPM). Later, a mixer module determines the final result for each ROI based on all the classification results. Fade \cite{steux2002fade} fuses monocular color vision and a RADAR data for vehicle detection and tracking. It is based on a belief network that checks the correlations between proposals from camera and vision, and determines which observations were wrong. Alessandretti at el. \cite{alessandretti2007vehicle} proposed a RADAR and camera fusion based approach for detecting guard rails and vehicles. In the proposed approach, ROIs are first located using RADAR data first. Then, vehicle detection algorithm is based on symmetry within the ROIs. Lekic at el. \cite{lekic2019automotive} proposed a Conditional Multi-Generator Generative Adversarial Network (CMGGAN) for RADAR-camera fusion. The CMGGAN is conditioned on RADAR data and generates camera-like images containing all the environmental features as detected by the RADAR. Ji et al. \cite{Ji2008} proposed a automotive RADAR and vision fusion for object classification (vehicle vs. other objects). Here, RADAR based detections are used to focus attention to a few candidate images that are later processed for generating sparse representation of objects.

Additionally, there exist many devices for tracking human activity\cite{Li2017}, autonomous driving\cite{Cho2014}, and so on, which fuse acquired data from a variety of sensors, including camera and RADAR, to achieve their results. We distinguish ourselves from this body of work by seeking to improve beyond filling complementary gaps that exist in RADARs and cameras, and that we iterate over processing for RADAR and cameras to improve images rather than fusing results obtained from each individual sensor. 

\textbf{Depth Completion:} 
